Supervised Feature Selection via Dependence Estimation

We introduce a framework for filtering features that employs the Hilbert-Schmidt Independence Criterion (HSIC) as a measure of dependence between the features and the labels. The key idea is that good features should maximise such dependence. Feature selection for various supervised learning problems (including classification and regression) is unified under this framework, and the solutions can be approximated using a backward-elimination algorithm. We demonstrate the usefulness of our method on both artificial and real world datasets.

==> Definitions.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{bm}

%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\DeclareMathOperator{\alphab}{\boldsymbol{\alpha}}

\DeclareMathOperator{\ab}{\mathbf{a}}
\DeclareMathOperator{\bb}{\mathbf{b}}
\DeclareMathOperator{\cbb}{\mathbf{c}}
\DeclareMathOperator{\db}{\mathbf{d}}
\DeclareMathOperator{\eb}{\mathbf{e}}
\DeclareMathOperator{\fb}{\mathbf{f}}
\DeclareMathOperator{\gb}{\mathbf{g}}
\DeclareMathOperator{\hb}{\mathbf{h}}
\DeclareMathOperator{\ib}{\mathbf{i}}
\DeclareMathOperator{\jb}{\mathbf{j}}
\DeclareMathOperator{\kb}{\mathbf{k}}
\DeclareMathOperator{\lb}{\mathbf{l}}
\DeclareMathOperator{\mb}{\mathbf{m}}
\DeclareMathOperator{\nbb}{\mathbf{n}}
\DeclareMathOperator{\ob}{\mathbf{o}}
\DeclareMathOperator{\pb}{\mathbf{p}}
\DeclareMathOperator{\qb}{\mathbf{q}}
\DeclareMathOperator{\rb}{\mathbf{r}}
\DeclareMathOperator{\sbb}{\mathbf{s}}
\DeclareMathOperator{\tb}{\mathbf{t}}
\DeclareMathOperator{\ub}{\mathbf{u}}
\DeclareMathOperator{\vb}{\mathbf{v}}
\DeclareMathOperator{\wb}{\mathbf{w}}
\DeclareMathOperator{\xb}{\mathbf{x}}
\DeclareMathOperator{\yb}{\mathbf{y}}
\DeclareMathOperator{\zb}{\mathbf{z}}

\DeclareMathOperator{\atilde}{\tilde{\ab}}
\DeclareMathOperator{\btilde}{\tilde{\bb}}
\DeclareMathOperator{\ctilde}{\tilde{\cbb}}
\DeclareMathOperator{\dtilde}{\tilde{\db}}
\DeclareMathOperator{\etilde}{\tilde{\eb}}
\DeclareMathOperator{\ftilde}{\tilde{\fb}}
\DeclareMathOperator{\gtilde}{\tilde{\gb}}
\DeclareMathOperator{\htilde}{\tilde{\hb}}
\DeclareMathOperator{\itilde}{\tilde{\ib}}
\DeclareMathOperator{\jtilde}{\tilde{\jb}}
\DeclareMathOperator{\ktilde}{\tilde{\kb}}
\DeclareMathOperator{\ltilde}{\tilde{\lb}}
\DeclareMathOperator{\mtilde}{\tilde{\mb}}
\DeclareMathOperator{\ntilde}{\tilde{\nbb}}
\DeclareMathOperator{\otilde}{\tilde{\ob}}
\DeclareMathOperator{\ptilde}{\tilde{\pb}}
\DeclareMathOperator{\qtilde}{\tilde{\qb}}
\DeclareMathOperator{\rtilde}{\tilde{\rb}}
\DeclareMathOperator{\stilde}{\tilde{\sbb}}
\DeclareMathOperator{\ttilde}{\tilde{\tb}}
\DeclareMathOperator{\utilde}{\tilde{\ub}}
\DeclareMathOperator{\vtilde}{\tilde{\vb}}
\DeclareMathOperator{\wtilde}{\tilde{\wb}}
\DeclareMathOperator{\xtilde}{\tilde{\xb}}
\DeclareMathOperator{\ytilde}{\tilde{\yb}}
\DeclareMathOperator{\ztilde}{\tilde{\zb}}

\DeclareMathOperator{\abar}{\bar{a}}
\DeclareMathOperator{\bbar}{\bar{b}}
\DeclareMathOperator{\cbar}{\bar{c}}
\DeclareMathOperator{\dbar}{\bar{d}}
\DeclareMathOperator{\ebar}{\bar{e}}
\DeclareMathOperator{\fbar}{\bar{f}}
\DeclareMathOperator{\gbar}{\bar{g}}
\DeclareMathOperator{\hbr}{\bar{h}}
\DeclareMathOperator{\ibar}{\bar{i}}
\DeclareMathOperator{\jbar}{\bar{j}}
\DeclareMathOperator{\kbar}{\bar{k}}
\DeclareMathOperator{\lbar}{\bar{l}}
\DeclareMathOperator{\mbar}{\bar{m}}
\DeclareMathOperator{\nbar}{\bar{n}}
\DeclareMathOperator{\obar}{\bar{o}}
\DeclareMathOperator{\pbar}{\bar{p}}
\DeclareMathOperator{\qbar}{\bar{q}}
\DeclareMathOperator{\rbar}{\bar{r}}
\DeclareMathOperator{\sbar}{\bar{s}}
\DeclareMathOperator{\tbar}{\bar{t}}
\DeclareMathOperator{\ubar}{\bar{u}}
\DeclareMathOperator{\vbar}{\bar{v}}
\DeclareMathOperator{\wbar}{\bar{w}}
\DeclareMathOperator{\xbar}{\bar{x}}
\DeclareMathOperator{\ybar}{\bar{y}}
\DeclareMathOperator{\zbar}{\bar{z}}

\DeclareMathOperator{\abbar}{\bar{\ab}}
\DeclareMathOperator{\bbbar}{\bar{\bb}}
\DeclareMathOperator{\cbbar}{\bar{\cb}}
\DeclareMathOperator{\dbbar}{\bar{\db}}
\DeclareMathOperator{\ebbar}{\bar{\eb}}
\DeclareMathOperator{\fbbar}{\bar{\fb}}
\DeclareMathOperator{\gbbar}{\bar{\gb}}
\DeclareMathOperator{\hbbar}{\bar{\hb}}
\DeclareMathOperator{\ibbar}{\bar{\ib}}
\DeclareMathOperator{\jbbar}{\bar{\jb}}
\DeclareMathOperator{\kbbar}{\bar{\kb}}
\DeclareMathOperator{\lbbar}{\bar{\lb}}
\DeclareMathOperator{\mbbar}{\bar{\mb}}
\DeclareMathOperator{\nbbar}{\bar{\nbb}}
\DeclareMathOperator{\obbar}{\bar{\ob}}
\DeclareMathOperator{\pbbar}{\bar{\pb}}
\DeclareMathOperator{\qbbar}{\bar{\qb}}
\DeclareMathOperator{\rbbar}{\bar{\rb}}
\DeclareMathOperator{\sbbar}{\bar{\sbb}}
\DeclareMathOperator{\tbbar}{\bar{\tb}}
\DeclareMathOperator{\ubbar}{\bar{\ub}}
\DeclareMathOperator{\vbbar}{\bar{\vb}}
\DeclareMathOperator{\wbbar}{\bar{\wb}}
\DeclareMathOperator{\xbbar}{\bar{\xb}}
\DeclareMathOperator{\ybbar}{\bar{\yb}}
\DeclareMathOperator{\zbbar}{\bar{\zb}}

\DeclareMathOperator{\Ab}{\mathbf{A}}
\DeclareMathOperator{\Bb}{\mathbf{B}}
\DeclareMathOperator{\Cb}{\mathbf{C}}
\DeclareMathOperator{\Db}{\mathbf{D}}
\DeclareMathOperator{\Eb}{\mathbf{E}}
\DeclareMathOperator{\Fb}{\mathbf{F}}
\DeclareMathOperator{\Gb}{\mathbf{G}}
\DeclareMathOperator{\Hb}{\mathbf{H}}
\DeclareMathOperator{\Ib}{\mathbf{I}}
\DeclareMathOperator{\Jb}{\mathbf{J}}
\DeclareMathOperator{\Kb}{\mathbf{K}}
\DeclareMathOperator{\Lb}{\mathbf{L}}
\DeclareMathOperator{\Mb}{\mathbf{M}}
\DeclareMathOperator{\Nb}{\mathbf{N}}
\DeclareMathOperator{\Ob}{\mathbf{O}}
\DeclareMathOperator{\Pb}{\mathbf{P}}
\DeclareMathOperator{\Qb}{\mathbf{Q}}
\DeclareMathOperator{\Rb}{\mathbf{R}}
\DeclareMathOperator{\Sbb}{\mathbf{S}}
\DeclareMathOperator{\Tb}{\mathbf{T}}
\DeclareMathOperator{\Ub}{\mathbf{U}}
\DeclareMathOperator{\Vb}{\mathbf{V}}
\DeclareMathOperator{\Wb}{\mathbf{W}}
\DeclareMathOperator{\Xb}{\mathbf{X}}
\DeclareMathOperator{\Yb}{\mathbf{Y}}
\DeclareMathOperator{\Zb}{\mathbf{Z}}

\DeclareMathOperator{\Abtil}{\tilde{\Ab}}
\DeclareMathOperator{\Bbtil}{\tilde{\Bb}}
\DeclareMathOperator{\Cbtil}{\tilde{\Cb}}
\DeclareMathOperator{\Dbtil}{\tilde{\Db}}
\DeclareMathOperator{\Ebtil}{\tilde{\Eb}}
\DeclareMathOperator{\Fbtil}{\tilde{\Fb}}
\DeclareMathOperator{\Gbtil}{\tilde{\Gb}}
\DeclareMathOperator{\Hbtil}{\tilde{\Hb}}
\DeclareMathOperator{\Ibtil}{\tilde{\Ib}}
\DeclareMathOperator{\Jbtil}{\tilde{\Jb}}
\DeclareMathOperator{\Kbtil}{\tilde{\Kb}}
\DeclareMathOperator{\Lbtil}{\tilde{\Lb}}
\DeclareMathOperator{\Mbtil}{\tilde{\Mb}}
\DeclareMathOperator{\Nbtil}{\tilde{\Nb}}
\DeclareMathOperator{\Obtil}{\tilde{\Ob}}
\DeclareMathOperator{\Pbtil}{\tilde{\Pb}}
\DeclareMathOperator{\Qbtil}{\tilde{\Qb}}
\DeclareMathOperator{\Rbtil}{\tilde{\Rb}}
\DeclareMathOperator{\Sbtil}{\tilde{\Sbb}}
\DeclareMathOperator{\Tbtil}{\tilde{\Tb}}
\DeclareMathOperator{\Ubtil}{\tilde{\Ub}}
\DeclareMathOperator{\Vbtil}{\tilde{\Vb}}
\DeclareMathOperator{\Wbtil}{\tilde{\Wb}}
\DeclareMathOperator{\Xbtil}{\tilde{\Xb}}
\DeclareMathOperator{\Ybtil}{\tilde{\Yb}}
\DeclareMathOperator{\Zbtil}{\tilde{\Zb}}

\DeclareMathOperator{\Abar}{\bar{A}}
\DeclareMathOperator{\Bbar}{\bar{B}}
\DeclareMathOperator{\Cbar}{\bar{C}}
\DeclareMathOperator{\Dbar}{\bar{D}}
\DeclareMathOperator{\Ebar}{\bar{E}}
\DeclareMathOperator{\Fbar}{\bar{F}}
\DeclareMathOperator{\Gbar}{\bar{G}}
\DeclareMathOperator{\Hbar}{\bar{H}}
\DeclareMathOperator{\Ibar}{\bar{I}}
\DeclareMathOperator{\Jbar}{\bar{J}}
\DeclareMathOperator{\Kbar}{\bar{K}}
\DeclareMathOperator{\Lbar}{\bar{L}}
\DeclareMathOperator{\Mbar}{\bar{M}}
\DeclareMathOperator{\Nbar}{\bar{N}}
\DeclareMathOperator{\Obar}{\bar{O}}
\DeclareMathOperator{\Pbar}{\bar{P}}
\DeclareMathOperator{\Qbar}{\bar{Q}}
\DeclareMathOperator{\Rbar}{\bar{R}}
\DeclareMathOperator{\Sbar}{\bar{S}}
\DeclareMathOperator{\Tbar}{\bar{T}}
\DeclareMathOperator{\Ubar}{\bar{U}}
\DeclareMathOperator{\Vbar}{\bar{V}}
\DeclareMathOperator{\Wbar}{\bar{W}}
\DeclareMathOperator{\Xbar}{\bar{X}}
\DeclareMathOperator{\Ybar}{\bar{Y}}
\DeclareMathOperator{\Zbar}{\bar{Z}}

\DeclareMathOperator{\Abbar}{\bar{\Ab}}
\DeclareMathOperator{\Bbbar}{\bar{\Bb}}
\DeclareMathOperator{\Cbbar}{\bar{\Cb}}
\DeclareMathOperator{\Dbbar}{\bar{\Db}}
\DeclareMathOperator{\Ebbar}{\bar{\Eb}}
\DeclareMathOperator{\Fbbar}{\bar{\Fb}}
\DeclareMathOperator{\Gbbar}{\bar{\Gb}}
\DeclareMathOperator{\Hbbar}{\bar{\Hb}}
\DeclareMathOperator{\Ibbar}{\bar{\Ib}}
\DeclareMathOperator{\Jbbar}{\bar{\Jb}}
\DeclareMathOperator{\Kbbar}{\bar{\Kb}}
\DeclareMathOperator{\Lbbar}{\bar{\Lb}}
\DeclareMathOperator{\Mbbar}{\bar{\Mb}}
\DeclareMathOperator{\Nbbar}{\bar{\Nb}}
\DeclareMathOperator{\Obbar}{\bar{\Ob}}
\DeclareMathOperator{\Pbbar}{\bar{\Pb}}
\DeclareMathOperator{\Qbbar}{\bar{\Qb}}
\DeclareMathOperator{\Rbbar}{\bar{\Rb}}
\DeclareMathOperator{\Sbbar}{\bar{\Sb}}
\DeclareMathOperator{\Tbbar}{\bar{\Tb}}
\DeclareMathOperator{\Ubbar}{\bar{\Ub}}
\DeclareMathOperator{\Vbbar}{\bar{\Vb}}
\DeclareMathOperator{\Wbbar}{\bar{\Wb}}
\DeclareMathOperator{\Xbbar}{\bar{\Xb}}
\DeclareMathOperator{\Ybbar}{\bar{\Yb}}
\DeclareMathOperator{\Zbbar}{\bar{\Zb}}

\DeclareMathOperator{\Ahat}{\hat{A}}
\DeclareMathOperator{\Bhat}{\hat{B}}
\DeclareMathOperator{\Chat}{\hat{C}}
\DeclareMathOperator{\Dhat}{\hat{D}}
\DeclareMathOperator{\Ehat}{\hat{E}}
\DeclareMathOperator{\Fhat}{\hat{F}}
\DeclareMathOperator{\Ghat}{\hat{G}}
\DeclareMathOperator{\Hhat}{\hat{H}}
\DeclareMathOperator{\Ihat}{\hat{I}}
\DeclareMathOperator{\Jhat}{\hat{J}}
\DeclareMathOperator{\Khat}{\hat{K}}
\DeclareMathOperator{\Lhat}{\hat{L}}
\DeclareMathOperator{\Mhat}{\hat{M}}
\DeclareMathOperator{\Nhat}{\hat{N}}
\DeclareMathOperator{\Ohat}{\hat{O}}
\DeclareMathOperator{\Phat}{\hat{P}}
\DeclareMathOperator{\Qhat}{\hat{Q}}
\DeclareMathOperator{\Rhat}{\hat{R}}
\DeclareMathOperator{\Shat}{\hat{S}}
\DeclareMathOperator{\That}{\hat{T}}
\DeclareMathOperator{\Uhat}{\hat{U}}
\DeclareMathOperator{\Vhat}{\hat{V}}
\DeclareMathOperator{\What}{\hat{W}}
\DeclareMathOperator{\Xhat}{\hat{X}}
\DeclareMathOperator{\Yhat}{\hat{Y}}
\DeclareMathOperator{\Zhat}{\hat{Z}}

\DeclareMathOperator{\Abhat}{\hat{\Ab}}
\DeclareMathOperator{\Bbhat}{\hat{\Bb}}
\DeclareMathOperator{\Cbhat}{\hat{\Cb}}
\DeclareMathOperator{\Dbhat}{\hat{\Db}}
\DeclareMathOperator{\Ebhat}{\hat{\Eb}}
\DeclareMathOperator{\Fbhat}{\hat{\Fb}}
\DeclareMathOperator{\Gbhat}{\hat{\Gb}}
\DeclareMathOperator{\Hbhat}{\hat{\Hb}}
\DeclareMathOperator{\Ibhat}{\hat{\Ib}}
\DeclareMathOperator{\Jbhat}{\hat{\Jb}}
\DeclareMathOperator{\Kbhat}{\hat{\Kb}}
\DeclareMathOperator{\Lbhat}{\hat{\Lb}}
\DeclareMathOperator{\Mbhat}{\hat{\Mb}}
\DeclareMathOperator{\Nbhat}{\hat{\Nb}}
\DeclareMathOperator{\Obhat}{\hat{\Ob}}
\DeclareMathOperator{\Pbhat}{\hat{\Pb}}
\DeclareMathOperator{\Qbhat}{\hat{\Qb}}
\DeclareMathOperator{\Rbhat}{\hat{\Rb}}
\DeclareMathOperator{\Sbhat}{\hat{\Sb}}
\DeclareMathOperator{\Tbhat}{\hat{\Tb}}
\DeclareMathOperator{\Ubhat}{\hat{\Ub}}
\DeclareMathOperator{\Vbhat}{\hat{\Vb}}
\DeclareMathOperator{\Wbhat}{\hat{\Wb}}
\DeclareMathOperator{\Xbhat}{\hat{\Xb}}
\DeclareMathOperator{\Ybhat}{\hat{\Yb}}
\DeclareMathOperator{\Zbhat}{\hat{\Zb}}

\DeclareMathOperator{\Acal}{\mathcal{A}}
\DeclareMathOperator{\Bcal}{\mathcal{B}}
\DeclareMathOperator{\Ccal}{\mathcal{C}}
\DeclareMathOperator{\Dcal}{\mathcal{D}}
\DeclareMathOperator{\Ecal}{\mathcal{E}}
\DeclareMathOperator{\Fcal}{\mathcal{F}}
\DeclareMathOperator{\Gcal}{\mathcal{G}}
\DeclareMathOperator{\Hcal}{\mathcal{H}}
\DeclareMathOperator{\Ical}{\mathcal{I}}
\DeclareMathOperator{\Jcal}{\mathcal{J}}
\DeclareMathOperator{\Kcal}{\mathcal{K}}
\DeclareMathOperator{\Lcal}{\mathcal{L}}
\DeclareMathOperator{\Mcal}{\mathcal{M}}
\DeclareMathOperator{\Ncal}{\mathcal{N}}
\DeclareMathOperator{\Ocal}{\mathcal{O}}
\DeclareMathOperator{\Pcal}{\mathcal{P}}
\DeclareMathOperator{\Qcal}{\mathcal{Q}}
\DeclareMathOperator{\Rcal}{\mathcal{R}}
\DeclareMathOperator{\Scal}{{\mathcal{S}}}
\DeclareMathOperator{\Tcal}{{\mathcal{T}}}
\DeclareMathOperator{\Ucal}{\mathcal{U}}
\DeclareMathOperator{\Vcal}{\mathcal{V}}
\DeclareMathOperator{\Wcal}{\mathcal{W}}
\DeclareMathOperator{\Xcal}{\mathcal{X}}
\DeclareMathOperator{\Ycal}{\mathcal{Y}}
\DeclareMathOperator{\Zcal}{\mathcal{Z}}

\DeclareMathOperator{\Atilde}{\widetilde{A}}
\DeclareMathOperator{\Btilde}{\widetilde{B}}
\DeclareMathOperator{\Ctilde}{\widetilde{C}}
\DeclareMathOperator{\Dtilde}{\widetilde{D}}
\DeclareMathOperator{\Etilde}{\widetilde{E}}
\DeclareMathOperator{\Ftilde}{\widetilde{F}}
\DeclareMathOperator{\Gtilde}{\widetilde{G}}
\DeclareMathOperator{\Htilde}{\widetilde{H}}
\DeclareMathOperator{\Itilde}{\widetilde{I}}
\DeclareMathOperator{\Jtilde}{\widetilde{J}}
\DeclareMathOperator{\Ktilde}{\widetilde{K}}
\DeclareMathOperator{\Ltilde}{\widetilde{L}}
\DeclareMathOperator{\Mtilde}{\widetilde{M}}
\DeclareMathOperator{\Ntilde}{\widetilde{N}}
\DeclareMathOperator{\Otilde}{\widetilde{O}}
\DeclareMathOperator{\Ptilde}{\widetilde{P}}
\DeclareMathOperator{\Qtilde}{\widetilde{Q}}
\DeclareMathOperator{\Rtilde}{\widetilde{R}}
\DeclareMathOperator{\Stilde}{\widetilde{S}}
\DeclareMathOperator{\Ttilde}{\widetilde{T}}
\DeclareMathOperator{\Utilde}{\widetilde{U}}
\DeclareMathOperator{\Vtilde}{\widetilde{V}}
\DeclareMathOperator{\Wtilde}{\widetilde{W}}
\DeclareMathOperator{\Xtilde}{\widetilde{X}}
\DeclareMathOperator{\Ytilde}{\widetilde{Y}}
\DeclareMathOperator{\Ztilde}{\widetilde{Z}}


%%%%%%%% Widely accepted definitions %%%%%%%%%%%%%%%

\DeclareMathOperator{\CC}{\mathbb{C}} % Complex numbers
\DeclareMathOperator{\EE}{\mathbb{E}} % Expectation
\DeclareMathOperator{\KK}{\mathbb{K}} % Arbitrary field
\DeclareMathOperator{\MM}{\mathbb{M}} % Median
\DeclareMathOperator{\NN}{\mathbb{N}} % Natural numbers
\DeclareMathOperator{\PP}{\mathbb{P}} % Probability
\DeclareMathOperator{\QQ}{\mathbb{Q}} % Rationals
\DeclareMathOperator{\RR}{\mathbb{R}} % Real numbers
\DeclareMathOperator{\ZZ}{\mathbb{Z}} % Integers

\DeclareMathOperator{\one}{\mathbf{1}}  % Identity
\DeclareMathOperator{\zero}{\mathbf{0}} % Zero
%\DeclareMathOperator{\TRUE}{\mathbf{TRUE}}  % True
%\DeclareMathOperator{\FALSE}{\mathbf{FALSE}}  % False

\DeclareMathOperator*{\mini}{\mathop{\mathrm{minimize}}}
\DeclareMathOperator*{\maxi}{\mathop{\mathrm{maximize}}}
\DeclareMathOperator*{\argmin}{\mathop{\mathrm{argmin}}}
\DeclareMathOperator*{\argmax}{\mathop{\mathrm{argmax}}}
\DeclareMathOperator{\sgn}{\mathop{\mathrm{sign}}}
\DeclareMathOperator{\tr}{\mathop{\mathrm{tr}}}
\DeclareMathOperator{\diag}{\mathop{\mathrm{diag}}}
\DeclareMathOperator{\rank}{\mathop{\mathrm{rank}}}
\DeclareMathOperator{\ovec}{\mathop{\mathrm{vec}}}
\DeclareMathOperator{\traj}{\mathop{\mathrm{Traj}}}
\DeclareMathOperator*{\cov}{\mathrm{Cov}}
\DeclareMathOperator*{\conv}{\mathrm{conv}}
\DeclareMathOperator*{\const}{\mathrm{constant}}

%%%%%%%% Bold Greek Letters %%%%%%%%%%%%%%%
\DeclareMathOperator{\sigmab}{\bm{\sigma}}
\DeclareMathOperator{\Sigmab}{\mathbf{\Sigma}}


%%%%%%%% Mess around with LaTeX %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
%\newenvironment{proof}{\emph{Proof. }}{ \hfill \QED}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\sembrack}[1]{[\![#1]\!]}

\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{i.i.d.}}

\newcommand{\alex}[1]{{\bf ALEX: \uppercase{#1}}}
\newcommand{\vishy}[1]{{\bf VISHY: \uppercase{#1}}}
\newcommand{\rene}[1]{{\bf RENE: \uppercase{#1}}}
\newcommand{\karsten}[1]{{\bf KARSTEN: \uppercase{#1}}}

%%%%%%%% Specific symbols for this project %%%%%%%%%%%%%%%

\newcommand{\methodname}{KDE}
\newcommand{\ind}{\boldsymbol{\mathsf{I}}}

\newcommand{\hsic}{\mathrm{HSIC}}
\newcommand{\mmd}{\mathrm{MMD}}

%\newcommand{\tDiag}{\textsf{Diag}}
%\newcommand{\tTr}{\textsf{Tr}}
%\newcommand{\tE}{\textsf{E}}
%\newcommand{\tVec}{\textsf{Vec}}
%\newcommand{\tRank}{\textsf{Rank}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% math symbols and commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\eq}[1]{(\ref{#1})}
%\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}

%brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\renewcommand{\url}[1]{{\sffamily #1}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "./SIGMOD06/SIGMODB06.tex"
%%% End:

